Bridging the Gap: Categorizing Gravitational-Wave Events at the Transition Between Neutron Stars and Black Holes

We search for features in the mass distribution of detected compact binary coalescences which signify the transition between neutron stars and black holes. We analyze all gravitational wave detections by LIGO-Virgo-KAGRA made through the end of the first half of the third observing run, and find clear evidence for two different populations of compact objects based solely on gravitational wave data. We confidently (99.3%) find a steepening relative to a single power law describing neutron stars and low-mass black holes below $2.4^{+0.5}_{-0.5}\text{ M}_{\odot}$, which is consistent with many predictions for the maximum neutron star mass. We find suggestions of the purported lower mass gap between the most massive neutron stars and the least massive black holes, but are unable to conclusively resolve it with current data. If it exists, we find the lower mass gap's edges to lie at $2.2^{+0.7}_{-0.5}\text{ M}_{\odot}$ and $6.0^{+2.4}_{-1.4}\text{ M}_{\odot}$. We re-examine events that have been deemed "exceptional" by the LIGO-Virgo-KAGRA collaborations in the context of these features. We analyze GW190814 self-consistently in the context of the full population of compact binaries, finding support for its secondary to be either a neutron star or a lower mass gap object, consistent with previous claims. Our models are the first to accommodate this event, which is an outlier with respect to the binary black hole population. We find that GW200105 and GW200115 probe the edges of, and may have components within, the lower mass gap. As future data improve global population models, the classification of these events will also improve.

==> macro_data_A_0_mbreak_free.tex <==
\makeatletter\newcommand\brokenMatterMattersBinnedPairing[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@out{\{"param": \{"A": \{"median": 0.0, "mean": 0.0, "5th percentile": 0.0, "95th percentile": 0.0, "error plus": 0.0, "error minus": 0.0\}, "NSmin": \{"median": 1.2, "mean": 1.2, "5th percentile": 1.1, "95th percentile": 1.4, "error plus": 0.2, "error minus": 0.1\}, "NSmax": \{"median": 2.4, "mean": 2.4, "5th percentile": 1.9, "95th percentile": 2.9, "error plus": 0.5, "error minus": 0.5\}, "BHmin": \{"median": 6.2, "mean": 6.2, "5th percentile": 3.7, "95th percentile": 8.7, "error plus": 2.5, "error minus": 2.5\}, "BHmax": \{"median": 46.0, "mean": 46.0, "5th percentile": 37.0, "95th percentile": 58.0, "error plus": 12.0, "error minus": 9.0\}, "n0": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n1": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n2": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n3": \{"median": 5.2, "mean": 5.5, "5th percentile": 3.4, "95th percentile": 8.8, "error plus": 3.6, "error minus": 1.8\}, "mbreak": \{"median": 5.0, "mean": 5.0, "5th percentile": 5.0, "95th percentile": 5.0, "error plus": 0.0, "error minus": 0.0\}, "alpha\_1": \{"median": {-}5.4, "mean": {-}5.3, "5th percentile": {-}7.6, "95th percentile": {-}2.9, "error plus": 2.5, "error minus": 2.2\}, "alpha\_2": \{"median": {-}1.0, "mean": {-}1.0, "5th percentile": {-}1.4, "95th percentile": {-}0.64, "error plus": 0.36, "error minus": 0.4\}, "beta\_q\_1": \{"median": 0.79, "mean": 0.91, "5th percentile": 0.13, "95th percentile": 2.0, "error plus": 1.2, "error minus": 0.66\}, "beta\_q\_2": \{"median": 3.5, "mean": 3.6, "5th percentile": 1.9, "95th percentile": 5.5, "error plus": 2.0, "error minus": 1.6\}\}, "rate": \{"bns": \{"median": 490.0, "mean": 570.0, "5th percentile": 120.0, "95th percentile": 1300.0, "error plus": 810.0, "error minus": 370.0\}, "nsbh": \{"median": 110.0, "mean": 130.0, "5th percentile": 17.0, "95th percentile": 300.0, "error plus": 190.0, "error minus": 93.0\}, "bbh": \{"median": 32.0, "mean": 33.0, "5th percentile": 21.0, "95th percentile": 48.0, "error plus": 16.0, "error minus": 11.0\}, "mass\_gap": \{"median": 94.0, "mean": 98.0, "5th percentile": 44.0, "95th percentile": 170.0, "error plus": 76.0, "error minus": 50.0\}, "above\_mg": \{"median": 43.0, "mean": 44.0, "5th percentile": 20.0, "95th percentile": 74.0, "error plus": 31.0, "error minus": 23.0\}, "full": \{"median": 760.0, "mean": 830.0, "5th percentile": 280.0, "95th percentile": 1700.0, "error plus": 940.0, "error minus": 480.0\}\}, "prob\_in\_gap": \{"GW151226": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.06, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.06, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "GW170608": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.12, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.12, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "GW170817": \{"prob\_mass1\_in\_gap": 0.01, "prob\_mass2\_in\_gap": 0.0, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.01, "prob\_mass1\_NS": 0.99, "prob\_mass2\_NS": 1.0, "prob\_mass1\_or\_mass2\_NS": 1.0, "prob\_NSBH": 0.01\}, "GW200115": \{"prob\_mass1\_in\_gap": 0.63, "prob\_mass2\_in\_gap": 0.06, "prob\_mass1\_and\_mass2\_in\_gap": 0.06, "prob\_mass1\_or\_mass2\_in\_gap": 0.64, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.94, "prob\_mass1\_or\_mass2\_NS": 0.94, "prob\_NSBH": 0.94\}, "GW200105": \{"prob\_mass1\_in\_gap": 0.06, "prob\_mass2\_in\_gap": 0.12, "prob\_mass1\_and\_mass2\_in\_gap": 0.03, "prob\_mass1\_or\_mass2\_in\_gap": 0.15, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.88, "prob\_mass1\_or\_mass2\_NS": 0.88, "prob\_NSBH": 0.88\}, "S190720a": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.05, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.05, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "S190814bv": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.65, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.65, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.35, "prob\_mass1\_or\_mass2\_NS": 0.35, "prob\_NSBH": 0.35\}, "S190924h": \{"prob\_mass1\_in\_gap": 0.16, "prob\_mass2\_in\_gap": 0.63, "prob\_mass1\_and\_mass2\_in\_gap": 0.16, "prob\_mass1\_or\_mass2\_in\_gap": 0.63, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "S190425z": \{"prob\_mass1\_in\_gap": 0.1, "prob\_mass2\_in\_gap": 0.0, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.1, "prob\_mass1\_NS": 0.9, "prob\_mass2\_NS": 1.0, "prob\_mass1\_or\_mass2\_NS": 1.0, "prob\_NSBH": 0.09\}, "S190930s": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.06, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.06, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}\}, "SD\_ratios": \{"A0": 0.0, "A1": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\brokenMatterMattersBinnedPairing@out\brokenMatterMattersBinnedPairing@I\else\ifnum\pdfstrcmp{#1}{rate}=0\let\brokenMatterMattersBinnedPairing@out\brokenMatterMattersBinnedPairing@II\else\ifnum\pdfstrcmp{#1}{prob_in_gap}=0\let\brokenMatterMattersBinnedPairing@out\brokenMatterMattersBinnedPairing@III\else\ifnum\pdfstrcmp{#1}{SD_ratios}=0\let\brokenMatterMattersBinnedPairing@out\brokenMatterMattersBinnedPairing@IV\else\def\brokenMatterMattersBinnedPairing@out{??}\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@out}\newcommand\brokenMatterMattersBinnedPairing@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@I@out{\{"A": \{"median": 0.0, "mean": 0.0, "5th percentile": 0.0, "95th percentile": 0.0, "error plus": 0.0, "error minus": 0.0\}, "NSmin": \{"median": 1.2, "mean": 1.2, "5th percentile": 1.1, "95th percentile": 1.4, "error plus": 0.2, "error minus": 0.1\}, "NSmax": \{"median": 2.4, "mean": 2.4, "5th percentile": 1.9, "95th percentile": 2.9, "error plus": 0.5, "error minus": 0.5\}, "BHmin": \{"median": 6.2, "mean": 6.2, "5th percentile": 3.7, "95th percentile": 8.7, "error plus": 2.5, "error minus": 2.5\}, "BHmax": \{"median": 46.0, "mean": 46.0, "5th percentile": 37.0, "95th percentile": 58.0, "error plus": 12.0, "error minus": 9.0\}, "n0": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n1": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n2": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n3": \{"median": 5.2, "mean": 5.5, "5th percentile": 3.4, "95th percentile": 8.8, "error plus": 3.6, "error minus": 1.8\}, "mbreak": \{"median": 5.0, "mean": 5.0, "5th percentile": 5.0, "95th percentile": 5.0, "error plus": 0.0, "error minus": 0.0\}, "alpha\_1": \{"median": {-}5.4, "mean": {-}5.3, "5th percentile": {-}7.6, "95th percentile": {-}2.9, "error plus": 2.5, "error minus": 2.2\}, "alpha\_2": \{"median": {-}1.0, "mean": {-}1.0, "5th percentile": {-}1.4, "95th percentile": {-}0.64, "error plus": 0.36, "error minus": 0.4\}, "beta\_q\_1": \{"median": 0.79, "mean": 0.91, "5th percentile": 0.13, "95th percentile": 2.0, "error plus": 1.2, "error minus": 0.66\}, "beta\_q\_2": \{"median": 3.5, "mean": 3.6, "5th percentile": 1.9, "95th percentile": 5.5, "error plus": 2.0, "error minus": 1.6\}\}}\else\ifnum\pdfstrcmp{#1}{A}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@V\else\ifnum\pdfstrcmp{#1}{NSmin}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@VI\else\ifnum\pdfstrcmp{#1}{NSmax}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@VII\else\ifnum\pdfstrcmp{#1}{BHmin}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@VIII\else\ifnum\pdfstrcmp{#1}{BHmax}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@IX\else\ifnum\pdfstrcmp{#1}{n0}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@X\else\ifnum\pdfstrcmp{#1}{n1}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@XI\else\ifnum\pdfstrcmp{#1}{n2}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@XII\else\ifnum\pdfstrcmp{#1}{n3}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@XIII\else\ifnum\pdfstrcmp{#1}{mbreak}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@XIV\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@XV\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@XVI\else\ifnum\pdfstrcmp{#1}{beta_q_1}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@XVII\else\ifnum\pdfstrcmp{#1}{beta_q_2}=0\let\brokenMatterMattersBinnedPairing@I@out\brokenMatterMattersBinnedPairing@XVIII\else\def\brokenMatterMattersBinnedPairing@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@I@out}\newcommand\brokenMatterMattersBinnedPairing@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@II@out{\{"bns": \{"median": 490.0, "mean": 570.0, "5th percentile": 120.0, "95th percentile": 1300.0, "error plus": 810.0, "error minus": 370.0\}, "nsbh": \{"median": 110.0, "mean": 130.0, "5th percentile": 17.0, "95th percentile": 300.0, "error plus": 190.0, "error minus": 93.0\}, "bbh": \{"median": 32.0, "mean": 33.0, "5th percentile": 21.0, "95th percentile": 48.0, "error plus": 16.0, "error minus": 11.0\}, "mass\_gap": \{"median": 94.0, "mean": 98.0, "5th percentile": 44.0, "95th percentile": 170.0, "error plus": 76.0, "error minus": 50.0\}, "above\_mg": \{"median": 43.0, "mean": 44.0, "5th percentile": 20.0, "95th percentile": 74.0, "error plus": 31.0, "error minus": 23.0\}, "full": \{"median": 760.0, "mean": 830.0, "5th percentile": 280.0, "95th percentile": 1700.0, "error plus": 940.0, "error minus": 480.0\}\}}\else\ifnum\pdfstrcmp{#1}{bns}=0\let\brokenMatterMattersBinnedPairing@II@out\brokenMatterMattersBinnedPairing@XIX\else\ifnum\pdfstrcmp{#1}{nsbh}=0\let\brokenMatterMattersBinnedPairing@II@out\brokenMatterMattersBinnedPairing@XX\else\ifnum\pdfstrcmp{#1}{bbh}=0\let\brokenMatterMattersBinnedPairing@II@out\brokenMatterMattersBinnedPairing@XXI\else\ifnum\pdfstrcmp{#1}{mass_gap}=0\let\brokenMatterMattersBinnedPairing@II@out\brokenMatterMattersBinnedPairing@XXII\else\ifnum\pdfstrcmp{#1}{above_mg}=0\let\brokenMatterMattersBinnedPairing@II@out\brokenMatterMattersBinnedPairing@XXIII\else\ifnum\pdfstrcmp{#1}{full}=0\let\brokenMatterMattersBinnedPairing@II@out\brokenMatterMattersBinnedPairing@XXIV\else\def\brokenMatterMattersBinnedPairing@II@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@II@out}\newcommand\brokenMatterMattersBinnedPairing@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@III@out{\{"GW151226": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.06, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.06, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "GW170608": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.12, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.12, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "GW170817": \{"prob\_mass1\_in\_gap": 0.01, "prob\_mass2\_in\_gap": 0.0, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.01, "prob\_mass1\_NS": 0.99, "prob\_mass2\_NS": 1.0, "prob\_mass1\_or\_mass2\_NS": 1.0, "prob\_NSBH": 0.01\}, "GW200115": \{"prob\_mass1\_in\_gap": 0.63, "prob\_mass2\_in\_gap": 0.06, "prob\_mass1\_and\_mass2\_in\_gap": 0.06, "prob\_mass1\_or\_mass2\_in\_gap": 0.64, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.94, "prob\_mass1\_or\_mass2\_NS": 0.94, "prob\_NSBH": 0.94\}, "GW200105": \{"prob\_mass1\_in\_gap": 0.06, "prob\_mass2\_in\_gap": 0.12, "prob\_mass1\_and\_mass2\_in\_gap": 0.03, "prob\_mass1\_or\_mass2\_in\_gap": 0.15, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.88, "prob\_mass1\_or\_mass2\_NS": 0.88, "prob\_NSBH": 0.88\}, "S190720a": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.05, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.05, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "S190814bv": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.65, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.65, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.35, "prob\_mass1\_or\_mass2\_NS": 0.35, "prob\_NSBH": 0.35\}, "S190924h": \{"prob\_mass1\_in\_gap": 0.16, "prob\_mass2\_in\_gap": 0.63, "prob\_mass1\_and\_mass2\_in\_gap": 0.16, "prob\_mass1\_or\_mass2\_in\_gap": 0.63, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "S190425z": \{"prob\_mass1\_in\_gap": 0.1, "prob\_mass2\_in\_gap": 0.0, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.1, "prob\_mass1\_NS": 0.9, "prob\_mass2\_NS": 1.0, "prob\_mass1\_or\_mass2\_NS": 1.0, "prob\_NSBH": 0.09\}, "S190930s": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.06, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.06, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}\}}\else\ifnum\pdfstrcmp{#1}{GW151226}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXV\else\ifnum\pdfstrcmp{#1}{GW170608}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXVI\else\ifnum\pdfstrcmp{#1}{GW170817}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXVII\else\ifnum\pdfstrcmp{#1}{GW200115}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXVIII\else\ifnum\pdfstrcmp{#1}{GW200105}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXIX\else\ifnum\pdfstrcmp{#1}{S190720a}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXX\else\ifnum\pdfstrcmp{#1}{S190814bv}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXXI\else\ifnum\pdfstrcmp{#1}{S190924h}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXXII\else\ifnum\pdfstrcmp{#1}{S190425z}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXXIII\else\ifnum\pdfstrcmp{#1}{S190930s}=0\let\brokenMatterMattersBinnedPairing@III@out\brokenMatterMattersBinnedPairing@XXXIV\else\def\brokenMatterMattersBinnedPairing@III@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@III@out}\newcommand\brokenMatterMattersBinnedPairing@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@IV@out{\{"A0": 0.0, "A1": 0.0\}}\else\ifnum\pdfstrcmp{#1}{A0}=0\def\brokenMatterMattersBinnedPairing@IV@out{0.0}\else\ifnum\pdfstrcmp{#1}{A1}=0\def\brokenMatterMattersBinnedPairing@IV@out{0.0}\else\def\brokenMatterMattersBinnedPairing@IV@out{??}\fi\fi\fi\brokenMatterMattersBinnedPairing@IV@out}\newcommand\brokenMatterMattersBinnedPairing@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@V@out{\{"median": 0.0, "mean": 0.0, "5th percentile": 0.0, "95th percentile": 0.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@V@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@V@out{0.0}\else\def\brokenMatterMattersBinnedPairing@V@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@V@out}\newcommand\brokenMatterMattersBinnedPairing@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@VI@out{\{"median": 1.2, "mean": 1.2, "5th percentile": 1.1, "95th percentile": 1.4, "error plus": 0.2, "error minus": 0.1\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@VI@out{1.2}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@VI@out{1.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@VI@out{1.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@VI@out{1.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@VI@out{0.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@VI@out{0.1}\else\def\brokenMatterMattersBinnedPairing@VI@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@VI@out}\newcommand\brokenMatterMattersBinnedPairing@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@VII@out{\{"median": 2.4, "mean": 2.4, "5th percentile": 1.9, "95th percentile": 2.9, "error plus": 0.5, "error minus": 0.5\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@VII@out{2.4}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@VII@out{2.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@VII@out{1.9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@VII@out{2.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@VII@out{0.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@VII@out{0.5}\else\def\brokenMatterMattersBinnedPairing@VII@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@VII@out}\newcommand\brokenMatterMattersBinnedPairing@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@VIII@out{\{"median": 6.2, "mean": 6.2, "5th percentile": 3.7, "95th percentile": 8.7, "error plus": 2.5, "error minus": 2.5\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@VIII@out{6.2}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@VIII@out{6.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@VIII@out{3.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@VIII@out{8.7}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@VIII@out{2.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@VIII@out{2.5}\else\def\brokenMatterMattersBinnedPairing@VIII@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@VIII@out}\newcommand\brokenMatterMattersBinnedPairing@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@IX@out{\{"median": 46.0, "mean": 46.0, "5th percentile": 37.0, "95th percentile": 58.0, "error plus": 12.0, "error minus": 9.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@IX@out{46.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@IX@out{46.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@IX@out{37.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@IX@out{58.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@IX@out{12.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@IX@out{9.0}\else\def\brokenMatterMattersBinnedPairing@IX@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@IX@out}\newcommand\brokenMatterMattersBinnedPairing@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@X@out{\{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@X@out{50.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@X@out{50.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@X@out{50.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@X@out{50.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@X@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@X@out{0.0}\else\def\brokenMatterMattersBinnedPairing@X@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@X@out}\newcommand\brokenMatterMattersBinnedPairing@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XI@out{\{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XI@out{50.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XI@out{50.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XI@out{50.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XI@out{50.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XI@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XI@out{0.0}\else\def\brokenMatterMattersBinnedPairing@XI@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XI@out}\newcommand\brokenMatterMattersBinnedPairing@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XII@out{\{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XII@out{50.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XII@out{50.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XII@out{50.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XII@out{50.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XII@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XII@out{0.0}\else\def\brokenMatterMattersBinnedPairing@XII@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XII@out}\newcommand\brokenMatterMattersBinnedPairing@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XIII@out{\{"median": 5.2, "mean": 5.5, "5th percentile": 3.4, "95th percentile": 8.8, "error plus": 3.6, "error minus": 1.8\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XIII@out{5.2}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XIII@out{5.5}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XIII@out{3.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XIII@out{8.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XIII@out{3.6}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XIII@out{1.8}\else\def\brokenMatterMattersBinnedPairing@XIII@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XIII@out}\newcommand\brokenMatterMattersBinnedPairing@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XIV@out{\{"median": 5.0, "mean": 5.0, "5th percentile": 5.0, "95th percentile": 5.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XIV@out{5.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XIV@out{5.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XIV@out{5.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XIV@out{5.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XIV@out{0.0}\else\def\brokenMatterMattersBinnedPairing@XIV@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XIV@out}\newcommand\brokenMatterMattersBinnedPairing@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XV@out{\{"median": {-}5.4, "mean": {-}5.3, "5th percentile": {-}7.6, "95th percentile": {-}2.9, "error plus": 2.5, "error minus": 2.2\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XV@out{{-}5.4}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XV@out{{-}5.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XV@out{{-}7.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XV@out{{-}2.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XV@out{2.5}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XV@out{2.2}\else\def\brokenMatterMattersBinnedPairing@XV@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XV@out}\newcommand\brokenMatterMattersBinnedPairing@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XVI@out{\{"median": {-}1.0, "mean": {-}1.0, "5th percentile": {-}1.4, "95th percentile": {-}0.64, "error plus": 0.36, "error minus": 0.4\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XVI@out{{-}1.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XVI@out{{-}1.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XVI@out{{-}1.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XVI@out{{-}0.64}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XVI@out{0.36}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XVI@out{0.4}\else\def\brokenMatterMattersBinnedPairing@XVI@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XVI@out}\newcommand\brokenMatterMattersBinnedPairing@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XVII@out{\{"median": 0.79, "mean": 0.91, "5th percentile": 0.13, "95th percentile": 2.0, "error plus": 1.2, "error minus": 0.66\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XVII@out{0.79}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XVII@out{0.91}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XVII@out{0.13}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XVII@out{2.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XVII@out{1.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XVII@out{0.66}\else\def\brokenMatterMattersBinnedPairing@XVII@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XVII@out}\newcommand\brokenMatterMattersBinnedPairing@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XVIII@out{\{"median": 3.5, "mean": 3.6, "5th percentile": 1.9, "95th percentile": 5.5, "error plus": 2.0, "error minus": 1.6\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XVIII@out{3.5}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XVIII@out{3.6}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XVIII@out{1.9}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XVIII@out{5.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XVIII@out{2.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XVIII@out{1.6}\else\def\brokenMatterMattersBinnedPairing@XVIII@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XVIII@out}\newcommand\brokenMatterMattersBinnedPairing@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XIX@out{\{"median": 490.0, "mean": 570.0, "5th percentile": 120.0, "95th percentile": 1300.0, "error plus": 810.0, "error minus": 370.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XIX@out{490.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XIX@out{570.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XIX@out{120.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XIX@out{1300.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XIX@out{810.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XIX@out{370.0}\else\def\brokenMatterMattersBinnedPairing@XIX@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XIX@out}\newcommand\brokenMatterMattersBinnedPairing@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XX@out{\{"median": 110.0, "mean": 130.0, "5th percentile": 17.0, "95th percentile": 300.0, "error plus": 190.0, "error minus": 93.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XX@out{110.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XX@out{130.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XX@out{17.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XX@out{300.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XX@out{190.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XX@out{93.0}\else\def\brokenMatterMattersBinnedPairing@XX@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XX@out}\newcommand\brokenMatterMattersBinnedPairing@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXI@out{\{"median": 32.0, "mean": 33.0, "5th percentile": 21.0, "95th percentile": 48.0, "error plus": 16.0, "error minus": 11.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XXI@out{32.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XXI@out{33.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XXI@out{21.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XXI@out{48.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XXI@out{16.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XXI@out{11.0}\else\def\brokenMatterMattersBinnedPairing@XXI@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXI@out}\newcommand\brokenMatterMattersBinnedPairing@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXII@out{\{"median": 94.0, "mean": 98.0, "5th percentile": 44.0, "95th percentile": 170.0, "error plus": 76.0, "error minus": 50.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XXII@out{94.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XXII@out{98.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XXII@out{44.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XXII@out{170.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XXII@out{76.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XXII@out{50.0}\else\def\brokenMatterMattersBinnedPairing@XXII@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXII@out}\newcommand\brokenMatterMattersBinnedPairing@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXIII@out{\{"median": 43.0, "mean": 44.0, "5th percentile": 20.0, "95th percentile": 74.0, "error plus": 31.0, "error minus": 23.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XXIII@out{43.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XXIII@out{44.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XXIII@out{20.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XXIII@out{74.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XXIII@out{31.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XXIII@out{23.0}\else\def\brokenMatterMattersBinnedPairing@XXIII@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXIII@out}\newcommand\brokenMatterMattersBinnedPairing@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXIV@out{\{"median": 760.0, "mean": 830.0, "5th percentile": 280.0, "95th percentile": 1700.0, "error plus": 940.0, "error minus": 480.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\brokenMatterMattersBinnedPairing@XXIV@out{760.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\brokenMatterMattersBinnedPairing@XXIV@out{830.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\brokenMatterMattersBinnedPairing@XXIV@out{280.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\brokenMatterMattersBinnedPairing@XXIV@out{1700.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\brokenMatterMattersBinnedPairing@XXIV@out{940.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\brokenMatterMattersBinnedPairing@XXIV@out{480.0}\else\def\brokenMatterMattersBinnedPairing@XXIV@out{??}\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXIV@out}\newcommand\brokenMatterMattersBinnedPairing@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXV@out{\{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.06, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.06, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXV@out{0.06}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXV@out{0.06}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXV@out{0.0}\else\def\brokenMatterMattersBinnedPairing@XXV@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXV@out}\newcommand\brokenMatterMattersBinnedPairing@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXVI@out{\{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.12, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.12, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVI@out{0.12}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVI@out{0.12}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXVI@out{0.0}\else\def\brokenMatterMattersBinnedPairing@XXVI@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXVI@out}\newcommand\brokenMatterMattersBinnedPairing@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXVII@out{\{"prob\_mass1\_in\_gap": 0.01, "prob\_mass2\_in\_gap": 0.0, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.01, "prob\_mass1\_NS": 0.99, "prob\_mass2\_NS": 1.0, "prob\_mass1\_or\_mass2\_NS": 1.0, "prob\_NSBH": 0.01\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVII@out{0.01}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVII@out{0.01}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXVII@out{0.99}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXVII@out{1.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXVII@out{1.0}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXVII@out{0.01}\else\def\brokenMatterMattersBinnedPairing@XXVII@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXVII@out}\newcommand\brokenMatterMattersBinnedPairing@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXVIII@out{\{"prob\_mass1\_in\_gap": 0.63, "prob\_mass2\_in\_gap": 0.06, "prob\_mass1\_and\_mass2\_in\_gap": 0.06, "prob\_mass1\_or\_mass2\_in\_gap": 0.64, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.94, "prob\_mass1\_or\_mass2\_NS": 0.94, "prob\_NSBH": 0.94\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVIII@out{0.63}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVIII@out{0.06}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVIII@out{0.06}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXVIII@out{0.64}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXVIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXVIII@out{0.94}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXVIII@out{0.94}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXVIII@out{0.94}\else\def\brokenMatterMattersBinnedPairing@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXVIII@out}\newcommand\brokenMatterMattersBinnedPairing@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXIX@out{\{"prob\_mass1\_in\_gap": 0.06, "prob\_mass2\_in\_gap": 0.12, "prob\_mass1\_and\_mass2\_in\_gap": 0.03, "prob\_mass1\_or\_mass2\_in\_gap": 0.15, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.88, "prob\_mass1\_or\_mass2\_NS": 0.88, "prob\_NSBH": 0.88\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXIX@out{0.06}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXIX@out{0.12}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXIX@out{0.03}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXIX@out{0.15}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXIX@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXIX@out{0.88}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXIX@out{0.88}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXIX@out{0.88}\else\def\brokenMatterMattersBinnedPairing@XXIX@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXIX@out}\newcommand\brokenMatterMattersBinnedPairing@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXX@out{\{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.05, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.05, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXX@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXX@out{0.05}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXX@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXX@out{0.05}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXX@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXX@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXX@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXX@out{0.0}\else\def\brokenMatterMattersBinnedPairing@XXX@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXX@out}\newcommand\brokenMatterMattersBinnedPairing@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXXI@out{\{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.65, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.65, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.35, "prob\_mass1\_or\_mass2\_NS": 0.35, "prob\_NSBH": 0.35\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXI@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXI@out{0.65}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXI@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXI@out{0.65}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXXI@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXXI@out{0.35}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXXI@out{0.35}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXXI@out{0.35}\else\def\brokenMatterMattersBinnedPairing@XXXI@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXXI@out}\newcommand\brokenMatterMattersBinnedPairing@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXXII@out{\{"prob\_mass1\_in\_gap": 0.16, "prob\_mass2\_in\_gap": 0.63, "prob\_mass1\_and\_mass2\_in\_gap": 0.16, "prob\_mass1\_or\_mass2\_in\_gap": 0.63, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXII@out{0.16}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXII@out{0.63}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXII@out{0.16}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXII@out{0.63}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXXII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXXII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXXII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXXII@out{0.0}\else\def\brokenMatterMattersBinnedPairing@XXXII@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXXII@out}\newcommand\brokenMatterMattersBinnedPairing@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXXIII@out{\{"prob\_mass1\_in\_gap": 0.1, "prob\_mass2\_in\_gap": 0.0, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.1, "prob\_mass1\_NS": 0.9, "prob\_mass2\_NS": 1.0, "prob\_mass1\_or\_mass2\_NS": 1.0, "prob\_NSBH": 0.09\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXIII@out{0.1}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXIII@out{0.1}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXXIII@out{0.9}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXXIII@out{1.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXXIII@out{1.0}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXXIII@out{0.09}\else\def\brokenMatterMattersBinnedPairing@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXXIII@out}\newcommand\brokenMatterMattersBinnedPairing@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\brokenMatterMattersBinnedPairing@XXXIV@out{\{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.06, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.06, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXIV@out{0.06}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\brokenMatterMattersBinnedPairing@XXXIV@out{0.06}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\brokenMatterMattersBinnedPairing@XXXIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXXIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\brokenMatterMattersBinnedPairing@XXXIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\brokenMatterMattersBinnedPairing@XXXIV@out{0.0}\else\def\brokenMatterMattersBinnedPairing@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\brokenMatterMattersBinnedPairing@XXXIV@out}\makeatother


==> macro_data_mbreak_is_gammalow.tex <==
\makeatletter\newcommand\dipbreakMatterMattersBinnedPairing[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@out{\{"param": \{"A": \{"median": 0.84, "mean": 0.79, "5th percentile": 0.42, "95th percentile": 0.98, "error plus": 0.14, "error minus": 0.42\}, "NSmin": \{"median": 1.2, "mean": 1.2, "5th percentile": 1.0, "95th percentile": 1.3, "error plus": 0.1, "error minus": 0.2\}, "NSmax": \{"median": 2.2, "mean": 2.3, "5th percentile": 1.7, "95th percentile": 2.9, "error plus": 0.7, "error minus": 0.5\}, "BHmin": \{"median": 6.0, "mean": 6.2, "5th percentile": 4.6, "95th percentile": 8.4, "error plus": 2.4, "error minus": 1.4\}, "BHmax": \{"median": 51.0, "mean": 52.0, "5th percentile": 40.0, "95th percentile": 69.0, "error plus": 18.0, "error minus": 11.0\}, "n0": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n1": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n2": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n3": \{"median": 5.4, "mean": 5.8, "5th percentile": 3.1, "95th percentile": 9.6, "error plus": 4.2, "error minus": 2.3\}, "mbreak": \{"median": 5.0, "mean": 5.0, "5th percentile": 5.0, "95th percentile": 5.0, "error plus": 0.0, "error minus": 0.0\}, "alpha\_1": \{"median": {-}3.8, "mean": {-}3.8, "5th percentile": {-}6.8, "95th percentile": {-}0.8, "error plus": 3.0, "error minus": 3.0\}, "alpha\_2": \{"median": {-}1.3, "mean": {-}1.3, "5th percentile": {-}1.8, "95th percentile": {-}0.92, "error plus": 0.38, "error minus": 0.5\}, "beta\_q\_1": \{"median": 0.59, "mean": 0.67, "5th percentile": 0.1, "95th percentile": 1.5, "error plus": 0.91, "error minus": 0.49\}, "beta\_q\_2": \{"median": 4.2, "mean": 4.4, "5th percentile": 2.3, "95th percentile": 7.1, "error plus": 2.9, "error minus": 1.9\}\}, "rate": \{"bns": \{"median": 460.0, "mean": 550.0, "5th percentile": 120.0, "95th percentile": 1300.0, "error plus": 840.0, "error minus": 340.0\}, "nsbh": \{"median": 170.0, "mean": 180.0, "5th percentile": 41.0, "95th percentile": 350.0, "error plus": 180.0, "error minus": 130.0\}, "bbh": \{"median": 37.0, "mean": 38.0, "5th percentile": 25.0, "95th percentile": 56.0, "error plus": 19.0, "error minus": 12.0\}, "mass\_gap": \{"median": 37.0, "mean": 44.0, "5th percentile": 5.7, "95th percentile": 110.0, "error plus": 73.0, "error minus": 31.0\}, "above\_mg": \{"median": 38.0, "mean": 41.0, "5th percentile": 9.4, "95th percentile": 83.0, "error plus": 45.0, "error minus": 29.0\}, "full": \{"median": 730.0, "mean": 810.0, "5th percentile": 320.0, "95th percentile": 1600.0, "error plus": 870.0, "error minus": 410.0\}\}, "prob\_in\_gap": \{"GW170817": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.0, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.0, "prob\_mass1\_NS": 1.0, "prob\_mass2\_NS": 1.0, "prob\_mass1\_or\_mass2\_NS": 1.0, "prob\_NSBH": 0.0\}, "GW200115": \{"prob\_mass1\_in\_gap": 0.44, "prob\_mass2\_in\_gap": 0.04, "prob\_mass1\_and\_mass2\_in\_gap": 0.03, "prob\_mass1\_or\_mass2\_in\_gap": 0.44, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.96, "prob\_mass1\_or\_mass2\_NS": 0.96, "prob\_NSBH": 0.96\}, "GW200105": \{"prob\_mass1\_in\_gap": 0.02, "prob\_mass2\_in\_gap": 0.19, "prob\_mass1\_and\_mass2\_in\_gap": 0.01, "prob\_mass1\_or\_mass2\_in\_gap": 0.19, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.81, "prob\_mass1\_or\_mass2\_NS": 0.81, "prob\_NSBH": 0.81\}, "S190814bv": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.74, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.74, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.26, "prob\_mass1\_or\_mass2\_NS": 0.26, "prob\_NSBH": 0.26\}, "S190924h": \{"prob\_mass1\_in\_gap": 0.05, "prob\_mass2\_in\_gap": 0.49, "prob\_mass1\_and\_mass2\_in\_gap": 0.05, "prob\_mass1\_or\_mass2\_in\_gap": 0.49, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "S190425z": \{"prob\_mass1\_in\_gap": 0.13, "prob\_mass2\_in\_gap": 0.01, "prob\_mass1\_and\_mass2\_in\_gap": 0.01, "prob\_mass1\_or\_mass2\_in\_gap": 0.13, "prob\_mass1\_NS": 0.87, "prob\_mass2\_NS": 0.99, "prob\_mass1\_or\_mass2\_NS": 0.99, "prob\_NSBH": 0.13\}\}, "SD\_ratios": \{"A0": 0.0387, "A1": 2.13\}\}}\else\ifnum\pdfstrcmp{#1}{param}=0\let\dipbreakMatterMattersBinnedPairing@out\dipbreakMatterMattersBinnedPairing@I\else\ifnum\pdfstrcmp{#1}{rate}=0\let\dipbreakMatterMattersBinnedPairing@out\dipbreakMatterMattersBinnedPairing@II\else\ifnum\pdfstrcmp{#1}{prob_in_gap}=0\let\dipbreakMatterMattersBinnedPairing@out\dipbreakMatterMattersBinnedPairing@III\else\ifnum\pdfstrcmp{#1}{SD_ratios}=0\let\dipbreakMatterMattersBinnedPairing@out\dipbreakMatterMattersBinnedPairing@IV\else\def\dipbreakMatterMattersBinnedPairing@out{??}\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@out}\newcommand\dipbreakMatterMattersBinnedPairing@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@I@out{\{"A": \{"median": 0.84, "mean": 0.79, "5th percentile": 0.42, "95th percentile": 0.98, "error plus": 0.14, "error minus": 0.42\}, "NSmin": \{"median": 1.2, "mean": 1.2, "5th percentile": 1.0, "95th percentile": 1.3, "error plus": 0.1, "error minus": 0.2\}, "NSmax": \{"median": 2.2, "mean": 2.3, "5th percentile": 1.7, "95th percentile": 2.9, "error plus": 0.7, "error minus": 0.5\}, "BHmin": \{"median": 6.0, "mean": 6.2, "5th percentile": 4.6, "95th percentile": 8.4, "error plus": 2.4, "error minus": 1.4\}, "BHmax": \{"median": 51.0, "mean": 52.0, "5th percentile": 40.0, "95th percentile": 69.0, "error plus": 18.0, "error minus": 11.0\}, "n0": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n1": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n2": \{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}, "n3": \{"median": 5.4, "mean": 5.8, "5th percentile": 3.1, "95th percentile": 9.6, "error plus": 4.2, "error minus": 2.3\}, "mbreak": \{"median": 5.0, "mean": 5.0, "5th percentile": 5.0, "95th percentile": 5.0, "error plus": 0.0, "error minus": 0.0\}, "alpha\_1": \{"median": {-}3.8, "mean": {-}3.8, "5th percentile": {-}6.8, "95th percentile": {-}0.8, "error plus": 3.0, "error minus": 3.0\}, "alpha\_2": \{"median": {-}1.3, "mean": {-}1.3, "5th percentile": {-}1.8, "95th percentile": {-}0.92, "error plus": 0.38, "error minus": 0.5\}, "beta\_q\_1": \{"median": 0.59, "mean": 0.67, "5th percentile": 0.1, "95th percentile": 1.5, "error plus": 0.91, "error minus": 0.49\}, "beta\_q\_2": \{"median": 4.2, "mean": 4.4, "5th percentile": 2.3, "95th percentile": 7.1, "error plus": 2.9, "error minus": 1.9\}\}}\else\ifnum\pdfstrcmp{#1}{A}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@V\else\ifnum\pdfstrcmp{#1}{NSmin}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@VI\else\ifnum\pdfstrcmp{#1}{NSmax}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@VII\else\ifnum\pdfstrcmp{#1}{BHmin}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@VIII\else\ifnum\pdfstrcmp{#1}{BHmax}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@IX\else\ifnum\pdfstrcmp{#1}{n0}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@X\else\ifnum\pdfstrcmp{#1}{n1}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@XI\else\ifnum\pdfstrcmp{#1}{n2}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@XII\else\ifnum\pdfstrcmp{#1}{n3}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@XIII\else\ifnum\pdfstrcmp{#1}{mbreak}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@XIV\else\ifnum\pdfstrcmp{#1}{alpha_1}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@XV\else\ifnum\pdfstrcmp{#1}{alpha_2}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@XVI\else\ifnum\pdfstrcmp{#1}{beta_q_1}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@XVII\else\ifnum\pdfstrcmp{#1}{beta_q_2}=0\let\dipbreakMatterMattersBinnedPairing@I@out\dipbreakMatterMattersBinnedPairing@XVIII\else\def\dipbreakMatterMattersBinnedPairing@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@I@out}\newcommand\dipbreakMatterMattersBinnedPairing@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@II@out{\{"bns": \{"median": 460.0, "mean": 550.0, "5th percentile": 120.0, "95th percentile": 1300.0, "error plus": 840.0, "error minus": 340.0\}, "nsbh": \{"median": 170.0, "mean": 180.0, "5th percentile": 41.0, "95th percentile": 350.0, "error plus": 180.0, "error minus": 130.0\}, "bbh": \{"median": 37.0, "mean": 38.0, "5th percentile": 25.0, "95th percentile": 56.0, "error plus": 19.0, "error minus": 12.0\}, "mass\_gap": \{"median": 37.0, "mean": 44.0, "5th percentile": 5.7, "95th percentile": 110.0, "error plus": 73.0, "error minus": 31.0\}, "above\_mg": \{"median": 38.0, "mean": 41.0, "5th percentile": 9.4, "95th percentile": 83.0, "error plus": 45.0, "error minus": 29.0\}, "full": \{"median": 730.0, "mean": 810.0, "5th percentile": 320.0, "95th percentile": 1600.0, "error plus": 870.0, "error minus": 410.0\}\}}\else\ifnum\pdfstrcmp{#1}{bns}=0\let\dipbreakMatterMattersBinnedPairing@II@out\dipbreakMatterMattersBinnedPairing@XIX\else\ifnum\pdfstrcmp{#1}{nsbh}=0\let\dipbreakMatterMattersBinnedPairing@II@out\dipbreakMatterMattersBinnedPairing@XX\else\ifnum\pdfstrcmp{#1}{bbh}=0\let\dipbreakMatterMattersBinnedPairing@II@out\dipbreakMatterMattersBinnedPairing@XXI\else\ifnum\pdfstrcmp{#1}{mass_gap}=0\let\dipbreakMatterMattersBinnedPairing@II@out\dipbreakMatterMattersBinnedPairing@XXII\else\ifnum\pdfstrcmp{#1}{above_mg}=0\let\dipbreakMatterMattersBinnedPairing@II@out\dipbreakMatterMattersBinnedPairing@XXIII\else\ifnum\pdfstrcmp{#1}{full}=0\let\dipbreakMatterMattersBinnedPairing@II@out\dipbreakMatterMattersBinnedPairing@XXIV\else\def\dipbreakMatterMattersBinnedPairing@II@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@II@out}\newcommand\dipbreakMatterMattersBinnedPairing@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@III@out{\{"GW170817": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.0, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.0, "prob\_mass1\_NS": 1.0, "prob\_mass2\_NS": 1.0, "prob\_mass1\_or\_mass2\_NS": 1.0, "prob\_NSBH": 0.0\}, "GW200115": \{"prob\_mass1\_in\_gap": 0.44, "prob\_mass2\_in\_gap": 0.04, "prob\_mass1\_and\_mass2\_in\_gap": 0.03, "prob\_mass1\_or\_mass2\_in\_gap": 0.44, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.96, "prob\_mass1\_or\_mass2\_NS": 0.96, "prob\_NSBH": 0.96\}, "GW200105": \{"prob\_mass1\_in\_gap": 0.02, "prob\_mass2\_in\_gap": 0.19, "prob\_mass1\_and\_mass2\_in\_gap": 0.01, "prob\_mass1\_or\_mass2\_in\_gap": 0.19, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.81, "prob\_mass1\_or\_mass2\_NS": 0.81, "prob\_NSBH": 0.81\}, "S190814bv": \{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.74, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.74, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.26, "prob\_mass1\_or\_mass2\_NS": 0.26, "prob\_NSBH": 0.26\}, "S190924h": \{"prob\_mass1\_in\_gap": 0.05, "prob\_mass2\_in\_gap": 0.49, "prob\_mass1\_and\_mass2\_in\_gap": 0.05, "prob\_mass1\_or\_mass2\_in\_gap": 0.49, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}, "S190425z": \{"prob\_mass1\_in\_gap": 0.13, "prob\_mass2\_in\_gap": 0.01, "prob\_mass1\_and\_mass2\_in\_gap": 0.01, "prob\_mass1\_or\_mass2\_in\_gap": 0.13, "prob\_mass1\_NS": 0.87, "prob\_mass2\_NS": 0.99, "prob\_mass1\_or\_mass2\_NS": 0.99, "prob\_NSBH": 0.13\}\}}\else\ifnum\pdfstrcmp{#1}{GW170817}=0\let\dipbreakMatterMattersBinnedPairing@III@out\dipbreakMatterMattersBinnedPairing@XXV\else\ifnum\pdfstrcmp{#1}{GW200115}=0\let\dipbreakMatterMattersBinnedPairing@III@out\dipbreakMatterMattersBinnedPairing@XXVI\else\ifnum\pdfstrcmp{#1}{GW200105}=0\let\dipbreakMatterMattersBinnedPairing@III@out\dipbreakMatterMattersBinnedPairing@XXVII\else\ifnum\pdfstrcmp{#1}{S190814bv}=0\let\dipbreakMatterMattersBinnedPairing@III@out\dipbreakMatterMattersBinnedPairing@XXVIII\else\ifnum\pdfstrcmp{#1}{S190924h}=0\let\dipbreakMatterMattersBinnedPairing@III@out\dipbreakMatterMattersBinnedPairing@XXIX\else\ifnum\pdfstrcmp{#1}{S190425z}=0\let\dipbreakMatterMattersBinnedPairing@III@out\dipbreakMatterMattersBinnedPairing@XXX\else\def\dipbreakMatterMattersBinnedPairing@III@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@III@out}\newcommand\dipbreakMatterMattersBinnedPairing@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@IV@out{\{"A0": 0.0387, "A1": 2.13\}}\else\ifnum\pdfstrcmp{#1}{A0}=0\def\dipbreakMatterMattersBinnedPairing@IV@out{0.0387}\else\ifnum\pdfstrcmp{#1}{A1}=0\def\dipbreakMatterMattersBinnedPairing@IV@out{2.13}\else\def\dipbreakMatterMattersBinnedPairing@IV@out{??}\fi\fi\fi\dipbreakMatterMattersBinnedPairing@IV@out}\newcommand\dipbreakMatterMattersBinnedPairing@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@V@out{\{"median": 0.84, "mean": 0.79, "5th percentile": 0.42, "95th percentile": 0.98, "error plus": 0.14, "error minus": 0.42\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@V@out{0.84}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@V@out{0.79}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@V@out{0.42}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@V@out{0.98}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@V@out{0.14}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@V@out{0.42}\else\def\dipbreakMatterMattersBinnedPairing@V@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@V@out}\newcommand\dipbreakMatterMattersBinnedPairing@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@VI@out{\{"median": 1.2, "mean": 1.2, "5th percentile": 1.0, "95th percentile": 1.3, "error plus": 0.1, "error minus": 0.2\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@VI@out{1.2}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@VI@out{1.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@VI@out{1.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@VI@out{1.3}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@VI@out{0.1}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@VI@out{0.2}\else\def\dipbreakMatterMattersBinnedPairing@VI@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@VI@out}\newcommand\dipbreakMatterMattersBinnedPairing@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@VII@out{\{"median": 2.2, "mean": 2.3, "5th percentile": 1.7, "95th percentile": 2.9, "error plus": 0.7, "error minus": 0.5\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@VII@out{2.2}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@VII@out{2.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@VII@out{1.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@VII@out{2.9}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@VII@out{0.7}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@VII@out{0.5}\else\def\dipbreakMatterMattersBinnedPairing@VII@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@VII@out}\newcommand\dipbreakMatterMattersBinnedPairing@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@VIII@out{\{"median": 6.0, "mean": 6.2, "5th percentile": 4.6, "95th percentile": 8.4, "error plus": 2.4, "error minus": 1.4\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@VIII@out{6.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@VIII@out{6.2}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@VIII@out{4.6}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@VIII@out{8.4}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@VIII@out{2.4}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@VIII@out{1.4}\else\def\dipbreakMatterMattersBinnedPairing@VIII@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@VIII@out}\newcommand\dipbreakMatterMattersBinnedPairing@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@IX@out{\{"median": 51.0, "mean": 52.0, "5th percentile": 40.0, "95th percentile": 69.0, "error plus": 18.0, "error minus": 11.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@IX@out{51.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@IX@out{52.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@IX@out{40.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@IX@out{69.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@IX@out{18.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@IX@out{11.0}\else\def\dipbreakMatterMattersBinnedPairing@IX@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@IX@out}\newcommand\dipbreakMatterMattersBinnedPairing@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@X@out{\{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@X@out{50.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@X@out{50.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@X@out{50.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@X@out{50.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@X@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@X@out{0.0}\else\def\dipbreakMatterMattersBinnedPairing@X@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@X@out}\newcommand\dipbreakMatterMattersBinnedPairing@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XI@out{\{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XI@out{50.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XI@out{50.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XI@out{50.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XI@out{50.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XI@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XI@out{0.0}\else\def\dipbreakMatterMattersBinnedPairing@XI@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XI@out}\newcommand\dipbreakMatterMattersBinnedPairing@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XII@out{\{"median": 50.0, "mean": 50.0, "5th percentile": 50.0, "95th percentile": 50.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XII@out{50.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XII@out{50.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XII@out{50.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XII@out{50.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XII@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XII@out{0.0}\else\def\dipbreakMatterMattersBinnedPairing@XII@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XII@out}\newcommand\dipbreakMatterMattersBinnedPairing@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XIII@out{\{"median": 5.4, "mean": 5.8, "5th percentile": 3.1, "95th percentile": 9.6, "error plus": 4.2, "error minus": 2.3\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XIII@out{5.4}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XIII@out{5.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XIII@out{3.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XIII@out{9.6}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XIII@out{4.2}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XIII@out{2.3}\else\def\dipbreakMatterMattersBinnedPairing@XIII@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XIII@out}\newcommand\dipbreakMatterMattersBinnedPairing@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XIV@out{\{"median": 5.0, "mean": 5.0, "5th percentile": 5.0, "95th percentile": 5.0, "error plus": 0.0, "error minus": 0.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XIV@out{5.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XIV@out{5.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XIV@out{5.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XIV@out{5.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XIV@out{0.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XIV@out{0.0}\else\def\dipbreakMatterMattersBinnedPairing@XIV@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XIV@out}\newcommand\dipbreakMatterMattersBinnedPairing@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XV@out{\{"median": {-}3.8, "mean": {-}3.8, "5th percentile": {-}6.8, "95th percentile": {-}0.8, "error plus": 3.0, "error minus": 3.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XV@out{{-}3.8}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XV@out{{-}3.8}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XV@out{{-}6.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XV@out{{-}0.8}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XV@out{3.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XV@out{3.0}\else\def\dipbreakMatterMattersBinnedPairing@XV@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XV@out}\newcommand\dipbreakMatterMattersBinnedPairing@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XVI@out{\{"median": {-}1.3, "mean": {-}1.3, "5th percentile": {-}1.8, "95th percentile": {-}0.92, "error plus": 0.38, "error minus": 0.5\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XVI@out{{-}1.3}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XVI@out{{-}1.3}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XVI@out{{-}1.8}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XVI@out{{-}0.92}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XVI@out{0.38}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XVI@out{0.5}\else\def\dipbreakMatterMattersBinnedPairing@XVI@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XVI@out}\newcommand\dipbreakMatterMattersBinnedPairing@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XVII@out{\{"median": 0.59, "mean": 0.67, "5th percentile": 0.1, "95th percentile": 1.5, "error plus": 0.91, "error minus": 0.49\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XVII@out{0.59}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XVII@out{0.67}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XVII@out{0.1}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XVII@out{1.5}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XVII@out{0.91}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XVII@out{0.49}\else\def\dipbreakMatterMattersBinnedPairing@XVII@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XVII@out}\newcommand\dipbreakMatterMattersBinnedPairing@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XVIII@out{\{"median": 4.2, "mean": 4.4, "5th percentile": 2.3, "95th percentile": 7.1, "error plus": 2.9, "error minus": 1.9\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XVIII@out{4.2}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XVIII@out{4.4}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XVIII@out{2.3}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XVIII@out{7.1}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XVIII@out{2.9}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XVIII@out{1.9}\else\def\dipbreakMatterMattersBinnedPairing@XVIII@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XVIII@out}\newcommand\dipbreakMatterMattersBinnedPairing@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XIX@out{\{"median": 460.0, "mean": 550.0, "5th percentile": 120.0, "95th percentile": 1300.0, "error plus": 840.0, "error minus": 340.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XIX@out{460.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XIX@out{550.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XIX@out{120.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XIX@out{1300.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XIX@out{840.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XIX@out{340.0}\else\def\dipbreakMatterMattersBinnedPairing@XIX@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XIX@out}\newcommand\dipbreakMatterMattersBinnedPairing@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XX@out{\{"median": 170.0, "mean": 180.0, "5th percentile": 41.0, "95th percentile": 350.0, "error plus": 180.0, "error minus": 130.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XX@out{170.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XX@out{180.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XX@out{41.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XX@out{350.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XX@out{180.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XX@out{130.0}\else\def\dipbreakMatterMattersBinnedPairing@XX@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XX@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXI@out{\{"median": 37.0, "mean": 38.0, "5th percentile": 25.0, "95th percentile": 56.0, "error plus": 19.0, "error minus": 12.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XXI@out{37.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XXI@out{38.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XXI@out{25.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XXI@out{56.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XXI@out{19.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XXI@out{12.0}\else\def\dipbreakMatterMattersBinnedPairing@XXI@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXI@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXII@out{\{"median": 37.0, "mean": 44.0, "5th percentile": 5.7, "95th percentile": 110.0, "error plus": 73.0, "error minus": 31.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XXII@out{37.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XXII@out{44.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XXII@out{5.7}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XXII@out{110.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XXII@out{73.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XXII@out{31.0}\else\def\dipbreakMatterMattersBinnedPairing@XXII@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXII@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXIII@out{\{"median": 38.0, "mean": 41.0, "5th percentile": 9.4, "95th percentile": 83.0, "error plus": 45.0, "error minus": 29.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XXIII@out{38.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XXIII@out{41.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XXIII@out{9.4}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XXIII@out{83.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XXIII@out{45.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XXIII@out{29.0}\else\def\dipbreakMatterMattersBinnedPairing@XXIII@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXIII@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXIV@out{\{"median": 730.0, "mean": 810.0, "5th percentile": 320.0, "95th percentile": 1600.0, "error plus": 870.0, "error minus": 410.0\}}\else\ifnum\pdfstrcmp{#1}{median}=0\def\dipbreakMatterMattersBinnedPairing@XXIV@out{730.0}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\dipbreakMatterMattersBinnedPairing@XXIV@out{810.0}\else\ifnum\pdfstrcmp{#1}{5th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XXIV@out{320.0}\else\ifnum\pdfstrcmp{#1}{95th percentile}=0\def\dipbreakMatterMattersBinnedPairing@XXIV@out{1600.0}\else\ifnum\pdfstrcmp{#1}{error plus}=0\def\dipbreakMatterMattersBinnedPairing@XXIV@out{870.0}\else\ifnum\pdfstrcmp{#1}{error minus}=0\def\dipbreakMatterMattersBinnedPairing@XXIV@out{410.0}\else\def\dipbreakMatterMattersBinnedPairing@XXIV@out{??}\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXIV@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXV@out{\{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.0, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.0, "prob\_mass1\_NS": 1.0, "prob\_mass2\_NS": 1.0, "prob\_mass1\_or\_mass2\_NS": 1.0, "prob\_NSBH": 0.0\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXV@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXV@out{1.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXV@out{1.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXV@out{1.0}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\dipbreakMatterMattersBinnedPairing@XXV@out{0.0}\else\def\dipbreakMatterMattersBinnedPairing@XXV@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXV@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXVI@out{\{"prob\_mass1\_in\_gap": 0.44, "prob\_mass2\_in\_gap": 0.04, "prob\_mass1\_and\_mass2\_in\_gap": 0.03, "prob\_mass1\_or\_mass2\_in\_gap": 0.44, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.96, "prob\_mass1\_or\_mass2\_NS": 0.96, "prob\_NSBH": 0.96\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVI@out{0.44}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVI@out{0.04}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVI@out{0.03}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVI@out{0.44}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXVI@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXVI@out{0.96}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXVI@out{0.96}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\dipbreakMatterMattersBinnedPairing@XXVI@out{0.96}\else\def\dipbreakMatterMattersBinnedPairing@XXVI@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXVI@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXVII@out{\{"prob\_mass1\_in\_gap": 0.02, "prob\_mass2\_in\_gap": 0.19, "prob\_mass1\_and\_mass2\_in\_gap": 0.01, "prob\_mass1\_or\_mass2\_in\_gap": 0.19, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.81, "prob\_mass1\_or\_mass2\_NS": 0.81, "prob\_NSBH": 0.81\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVII@out{0.02}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVII@out{0.19}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVII@out{0.01}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVII@out{0.19}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXVII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXVII@out{0.81}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXVII@out{0.81}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\dipbreakMatterMattersBinnedPairing@XXVII@out{0.81}\else\def\dipbreakMatterMattersBinnedPairing@XXVII@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXVII@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{\{"prob\_mass1\_in\_gap": 0.0, "prob\_mass2\_in\_gap": 0.74, "prob\_mass1\_and\_mass2\_in\_gap": 0.0, "prob\_mass1\_or\_mass2\_in\_gap": 0.74, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.26, "prob\_mass1\_or\_mass2\_NS": 0.26, "prob\_NSBH": 0.26\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{0.74}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{0.74}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{0.26}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{0.26}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{0.26}\else\def\dipbreakMatterMattersBinnedPairing@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXVIII@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXIX@out{\{"prob\_mass1\_in\_gap": 0.05, "prob\_mass2\_in\_gap": 0.49, "prob\_mass1\_and\_mass2\_in\_gap": 0.05, "prob\_mass1\_or\_mass2\_in\_gap": 0.49, "prob\_mass1\_NS": 0.0, "prob\_mass2\_NS": 0.0, "prob\_mass1\_or\_mass2\_NS": 0.0, "prob\_NSBH": 0.0\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXIX@out{0.05}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXIX@out{0.49}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXIX@out{0.05}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXIX@out{0.49}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXIX@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXIX@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXIX@out{0.0}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\dipbreakMatterMattersBinnedPairing@XXIX@out{0.0}\else\def\dipbreakMatterMattersBinnedPairing@XXIX@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXIX@out}\newcommand\dipbreakMatterMattersBinnedPairing@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\dipbreakMatterMattersBinnedPairing@XXX@out{\{"prob\_mass1\_in\_gap": 0.13, "prob\_mass2\_in\_gap": 0.01, "prob\_mass1\_and\_mass2\_in\_gap": 0.01, "prob\_mass1\_or\_mass2\_in\_gap": 0.13, "prob\_mass1\_NS": 0.87, "prob\_mass2\_NS": 0.99, "prob\_mass1\_or\_mass2\_NS": 0.99, "prob\_NSBH": 0.13\}}\else\ifnum\pdfstrcmp{#1}{prob_mass1_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXX@out{0.13}\else\ifnum\pdfstrcmp{#1}{prob_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXX@out{0.01}\else\ifnum\pdfstrcmp{#1}{prob_mass1_and_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXX@out{0.01}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_in_gap}=0\def\dipbreakMatterMattersBinnedPairing@XXX@out{0.13}\else\ifnum\pdfstrcmp{#1}{prob_mass1_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXX@out{0.87}\else\ifnum\pdfstrcmp{#1}{prob_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXX@out{0.99}\else\ifnum\pdfstrcmp{#1}{prob_mass1_or_mass2_NS}=0\def\dipbreakMatterMattersBinnedPairing@XXX@out{0.99}\else\ifnum\pdfstrcmp{#1}{prob_NSBH}=0\def\dipbreakMatterMattersBinnedPairing@XXX@out{0.13}\else\def\dipbreakMatterMattersBinnedPairing@XXX@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\dipbreakMatterMattersBinnedPairing@XXX@out}\makeatother

